Generate, Not Recommend: Personalized Multimodal Content Generation

To address the challenge of information overload from massive web contents, recommender systems are widely applied to retrieve and present personalized results for users. However, recommendation tasks are inherently constrained to filtering existing items and lack the ability to generate novel concepts, limiting their capacity to fully satisfy user demands and preferences. In this paper, we propose a new paradigm that goes beyond content filtering and selecting: directly generating personalized items in a multimodal form, such as images, tailored to individual users. To accomplish this, we leverage any-to-any Large Multimodal Models (LMMs) and train them in both supervised fine-tuning and online reinforcement learning strategy to equip them with the ability to yield tailored next items for users. Experiments on two benchmark datasets and user study confirm the efficacy of the proposed method. Notably, the generated images not only align well with users' historical preferences but also exhibit relevance to their potential future interests.

==> Related_Work.tex <==
\section{Related Work}
Existing works on personalized multimodal content generation mainly focus on situations that tailoring and customizing a reference candidate image based on the corresponding user histories. ~\cite{pmg,iamg} leverage LMMs to summarize history texts and images into profiles for the image generation module such stable diffusion to refer to. Recent studies~\cite{pig,drc} switch to produce latent and dense instruction embedding to guide the downstream image generation tasks. However, in this paper, we pay attention to the proactively image generation without any candidates and references. Furthermore, we utilize any-to-any LMMs to perform this personalized generation task in an end-to-end manner.
